Conformal Prediction and Human Decision Making

Methods to quantify uncertainty in predictions from arbitrary models are in demand in high-stakes domains like medicine and finance. Conformal prediction has emerged as a popular method for producing a set of predictions with specified average coverage, in place of a single prediction and confidence value. However, the value of conformal prediction sets to assist human decisions remains elusive due to the murky relationship between coverage guarantees and decision makers' goals and strategies. How should we think about conformal prediction sets as a form of decision support? We outline a decision theoretic framework for evaluating predictive uncertainty as informative signals, then contrast what can be said within this framework about idealized use of calibrated probabilities versus conformal prediction sets. Informed by prior empirical results and theories of human decisions under uncertainty, we formalize a set of possible strategies by which a decision maker might use a prediction set. We identify ways in which conformal prediction sets and posthoc predictive uncertainty quantification more broadly are in tension with common goals and needs in human-AI decision making. We give recommendations for future research in predictive uncertainty quantification to support human decision makers.

==> sections/06_01_aligned_uncertainty.tex <==
\section{Toward Human-Aligned Uncertainty Quantification}
\label{sec:humanuq}
%If twoishness is inherent in many applications of conformal uncertainty quantification for informing human decisions.

Our discussion above highlights several challenges to defining the value of conformal prediction sets for decision making. It is difficult to justify prediction sets from a decision theoretic perspective compared to measures of uncertainty that can be applied to specific predictions.
When end-users of the sets like human decision makers may have additional information, the guarantees are no longer interpretable in a straightforward way. 
Hence, theoretical guarantees do not necessarily capture the appeal of conformal prediction in practice. 

One might conclude from this discussion that conformal prediction sets are not worth pursuing as a general approach to quantifying prediction uncertainty, and that effort should instead be put on developing methods that can provide a measure of credibility at the level of individual predictions. 
However, this conclusion misses the point by assuming that theory, in this case formal justification from a decision making perspective, can explain the value of  quantified prediction uncertainty for human decision makers in practice. 


Like the bootstrap, split conformal prediction is widely applicable and conceptually simple. It provides a familiar form of uncertainty information (a confidence set).  
To understand its value, we must acknowledge that formal theory is not sufficient for characterizing the value of uncertainty in practice. When it comes to model-assisted human decisions, the meaning of quantified uncertainty is its use. This is not to say that the only knowledge we can gain is empirical though. Progress depends on acknowledging where gaps remain in our ability to understand and best design prediction sets, and using these gaps to motivate a science of human-aligned prediction uncertainty. We reflect on specific takeaways of our analysis toward this goal below.




\jessica{Section unfinished. High level takeaway:}

 It is natural to pursue theoretical analysis of new methods, thus we should not necessarily stop pursuing methods that allow us to achieve calibration over the right sources of randomness. However, we should expect our best attempts to still miss important things. Ultimately, what we can prove may have relatively little to do with the practical value of a method.

\jessica{stuff on decision calibration}


\jessica{More specific points I plan to make about conformal in this section:}
\begin{itemize}
    \item There is a silver lining to broadening our views on the value of a statistical method beyond theoretical guarantees: we are in a better position to recognize harder-to-formalize sources of practical value. 
    Some potentially useful information that we get with split conformal prediction is currently outside the bounds of theory or difficult to theorize at all. Even when we don't expect conformal coverage guarantees to hold exactly as stated (e.g., because of data shifts or constraints like spatial or temporal correlations, or additional knowledge a human possesses), information about model uncertainty captured in set size given adaptive techniques (e.g.,~\citep{angelopoulos2021uncertainty}) may still be valuable in many settings.
    \jessica{are there examples of using relative CI width for decisions even though coverage is not expected to be accurate?} \dawei{On the Expected Size of Conformal Prediction Sets ~\citep{dhillon2024expected}}
   
   \item  We should acknowledge that some aspects of human use of prediction sets are not easily amenable to any formalization, and therefore may remain important in practice but beyond our theories. For example, associational reasoning. A prediction set that does not contain the true label might still be useful to a human if the labels it does include prompt them to consider a broader set of possibilities and this leads them to identify the true label. 
   %Recent empirical work, for example, finds that even when test instances were drawn from a different distribution than calibration instances,  \citep{zhang2024} (
   
    \item Thus far the focus in the conformal lit has been on developing non-conformity scores. However, to align prediction sets with human needs may require paying more attention to the nature of the sets themselves. Better human decisions can often come from providing the decision maker with access to high-dimensional intermediate outputs from a model (e.g., a reconstructed version of a low-fidelity image). While some nascent work explores the construction of conformal prediction sets for such settings, little attention has been paid to whether the ``shape'' of the confidence sets in high dimensions aligns with what humans consider meaningful structures. Putting confidence sets on individual pixels in an image for example, may be less useful (and involve more problematic assumptions) than constructing sets at a coarser level aligned with human-meaningful features.

    \item Work showing that even calibrated model uncertainty information can lead a decision maker astray when they have access to different or additional features would seem to suggest multicalibrating uncertainty to both the model and the human's confidence functions~\citep{corvelo2024human} or otherwise re-mapping probabilities in ways that anticipate human use. But this remains incomplete in that we can overlook similar assumptions we must now make about humans to the original ones entailed by split conformal prediction (e.g., that they are exchangeable).
    What would it look like to normalize model-checking as a necessary part of any solution, where even with online solutions we are never done?
    
    
    \end{itemize}


\jessica{Somewhere here should be explicit about what aspects of our discussion apply to uncertainty quantification more broadly (like Frequentist CIs, Bayesian credible intervals)}







%\citep{lu2022fair} \url{https://arxiv.org/abs/2109.04392} - rule in and rule out dangerous conditions

%Using it to determine which instances a human expert should decide on

%Somewhere we should distinguish scenarios where the human has to make the final decision vs scenarios where you could make an automated decision (like if the prediction set was size 1)




\begin{comment}

\subsection{When can we define the value of a prediction set?}
We formalize the value of uncertainty in a model prediction to a decision problem using statistical decision theory, to illustrate why optimal use of a prediction set is under-determined. 

\jessica{Define decision problem (uncertain state, action space, scoring rule, optionally signals that inform about the payoff relevant state, captured by a data generating model}

For our purposes, a \textbf{decision problem} requires a decision maker to choose a response (\textbf{action}) $\action$ from some set of possible responses, or \textbf{action space}, $\actionspace$, where the quality of a decision depends on the \textbf{uncertain state} of the world $\mstate$, drawn from a finite, mutually exclusive \textbf{state space} $\statespace$. 
Model predictions provided to a decision maker represent a type of \textit{signal} that provide information to the decision maker about the state, generated by a \textbf{signaling policy} and associated with the uncertain state by the \textbf{data-generating model}, a distribution over values of the uncertain state and the signals. 
More formally, a signaling policy induces an \textbf{information
structure} that is given by a joint distribution $\joint \in \distover{\signalspace \times \statespace}$ over signals $\signal \in \signalspace$ and states $\mstate \in \statespace$.
This joint distribution assigns to each realization $(\signal,\mstate) \in \signalspace \times \statespace$ a
probability, denoted $\joint(\signal,\mstate)$.
The best action available to the decision maker is that which maxmizes the value of \textbf{scoring rule} in the decision problem, a function that assigns a score representing the quality of the action for the realized state.

%In decision tasks corresponding to prediction tasks,  the action space is a probabilistic belief over the state space, i.e., $\actionspace = \distover{\statespace}$. 

Under this definition, the formalization of the information structure $\joint$ enables a definition of normative behavior. 
Uncertainty information becomes relevant to the decision maker  because they must consider the probability of different states induced by the signal in order to choose best action under the scoring rule. 

\end{comment}


==> sections/06_twoishness.tex <==
\section{Epistemic uncertainty and the twoishness of statistical methods}
\label{sec:epistemic}
%An important selling point of split conformal prediction is that as a model-agnostic wrapper, it can be applied to arbitrarily-distributed data. 
There is a sharp contrast between calibrated prediction probabilities and prediction sets from the standpoint of specifying ideal decision strategies. However, it is important not to lose sight of the similarities between these approaches---as two examples of post hoc calibration---within the larger landscape of uncertainty quantification. In particular, reflecting on  the relationship between such methods and \textit{epistemic uncertainty} representing inherent limitations of our knowledge helps illustrate fundamental tradeoffs we encounter in quantifying uncertainty in blackbox predictions.  


Consider that offline calibration methods can often be described as relying on two models: the original black-box predictive model and the model of the frequency distribution of the predictions. 
Such ``twoishness'' is not entirely unique; rather, it is inherent in many statistical methods \citep{gelman2011}.  
For example, a common pattern occurs in classical statistical analysis, where one method is used to produce estimates (e.g., a multivariate regression to estimate effects and compute standard errors) and another is used to check if the first method makes sense (e.g., predictive checks or significance tests on the coefficients). 
%One could also consider tuning parameters in machine learning to be a form of twoishness, in that they can be set by the user independently of the model and allow more flexibility in implementation at the cost of losing coherence and calibration.


Split conformal prediction combines an arbitrary predictive model whose output we use to derive a non-conformity score as our data model (or likelihood) with a second model defined by the sampling distribution of the non-conformity scores.
%When a human decision maker and a predictive model have access to potentially differing information sets, uncertainty quantification based only on the model's information (or a separate calibration set) may be insufficient for good decisions, as it does not account for the human's model of the data-generating process. 
The benefits of combining these two models are obvious. 
We are absolved of having to understand the relationship between the model's training distribution and the deployment (test) distribution.
We can ignore that the original model may be misspecified, and focus on deriving prediction probabilities that hold on calibration data we choose.


However, twoishness also implies fundamental limitations to our ability to represent uncertainty. We reflect on this from the perspective of epistemic uncertainty about the appropriateness of assumptions, and provide an analogy to the standard bootstrap.

%we use an analogy to bootstrapping to illustrate several important gaps between theory and practice. We contrast second-order uncertainty with that provided by methods targeting calibration alone, and discuss why the former is sometimes undervalued in the literature. 

\subsection{Second-order uncertainty}
One way to understand what is lost when quantifying prediction uncertainty for black-box models draws on a common distinction between sources of risk and uncertainty. \textit{Aleatoric uncertainty}---uncertainty in an outcome due to inherent randomness in a process---is sometimes distinguished from \textit{epistemic uncertainty} due to a lack of knowledge that could in theory be reduced. While calibration offers assurance for good decisions under aleatoric uncertainty, its resolution of epistemic uncertainty is arguably less satisfying.


Continuing with multiclass classification as an example, a classifier $\model$ trained to minimize loss using a set of labeled training data can be thought of as producing predictions at different levels, which are evaluated using different empirical values. We can evaluate the ``level 0'' prediction $\ypredict = \model(\dataRV=\xb)$ of the label against the true label using 0/1 loss. We can evaluate the ``level 1'' prediction of the conditional distribution $\modelprob(\cdot|\dataRV=\xb)$ against the empirical distribution of labels. 


Aleatoric uncertainty captures the fact that even if we were given full knowledge of $p(\cdot|\dataRV=\xb)$, we cannot predict with certainty due to inherent randomness in the generating process. 
The ideal case for deploying a statistical predictor to make decisions is when we wish to minimize decision loss on average, and have access to a large amount of data that we are confident reflects the target generating process. In such cases, we are primarily concerned with aleatoric uncertainty. 


But what is the ideal case for post hoc calibration? The advantage of being able to calibrate a predictor post hoc implies that the original learning problem was misspecified with respect to our prediction goals: the learned probabilistic predictor $\modelprob$ associated with classifier $\model$ differs from the ground truth $p$. Distribution-free post hoc calibration of prediction uncertainty promises to ``fix'' the gap between $\modelprob$ and $p$, but offers the decision maker no information to estimate epistemic uncertainty, i.e., how different the prediction $\modelprob(\cdot|\dataRV=\xb)$ may be from the ground truth. The need to recalibrate makes clear that our assumptions may fail to capture reality, but leaves the representational gap unaddressed in an explicit way.


%When probability is defined as frequency, for describing epistemic uncertainty. 
Because we can't observe samples from the second order distribution $\mathbb{P}(\mathbb{P}(\ystate|\dataRV=\xb))$, we cannot learn a faithful predictor of higher order epistemic uncertainty within a loss minimization framework~\citep{bengs2022pitfalls}. This is formalized by \citet{bengs2023second}, who relate it to the impossibility of defining a proper scoring rule. Learning to predict conditional distributions $\modelprob(\cdot|\dataRV=\xb)$ using empirical risk minimization--i.e., identifying the empirical risk minimizer that minimizes loss on the training data---under a proper scoring rule means that the optimal predictor (the true risk minimizer or Bayes predictor) will coincide with the true conditional class distribution $\joint(\cdot|\dataRV=\xb)$. 
However, there is no loss function for comparing second-order predictions of $p(p(\cdot|\dataRV=\xb))$
with observations $\ystate$ such that minimizing that function on the training data ensures a second-order predictor will be ``honest'' in the sense of returning the prediction corresponding to its belief. 



We can contrast this with Bayesian probability, which can be distinguished from probability denoting expected frequency. 
When we specify priors on model parameters in a Bayesian model, we explicitly express this uncertainty in our predictions. 
The
posterior predictive distribution $p(y_{rep}|y)$ marginalizes the distribution of $y_{rep}$, which we can think of as a newly drawn version of $y$ given $\theta$, over the posterior distribution of $\theta$ given $y$, which, by virtue of conditioning the prior, captures epistemic uncertainty stemming from our lack of knowledge of the model parameters. 
In a machine learning context, the posterior predictive distribution of a Bayesian neural network with latent variables captures uncertainty in network weights as well as in random noise and latent variables in data generation~\citep{depeweg2018decomposition}.  


Rather than arguing for one statistical paradigm over another, our point here is simply that there is a risk to concluding that because higher order epistemic uncertainty cannot be directly evaluated, and is therefore of questionable value in a loss minimization framework, it cannot be useful for decision makers. Consider a situation where abstaining from making a decision in order to gather more information is possible. Offering the decision maker a probability distribution over the rate at which an event is expected to occur (as compared to a maximum likelihood point estimate) provides them a sense of how much risk is incurred by acting as if the maximum likelihood prediction is true versus holding out until more information is available. Similar to how we should consider what information is available to human decision-makers versus artificial agents when we design uncertainty quantification, we should also consider whether decision-makers would benefit from epistemic uncertainty that expresses the limitations of knowledge for a particular decision. This may be particularly desirable in situations where decision-makers are liable for individual decisions, such as about specific patients in a medical setting.



\subsection{The bootstrap as analogy}

%The need to prove guarantees on the calibration step can overshadow hard but important implementation questions. Often the guarantees will fail to capture why the techniques are used in practice.
%A lack of appreciation for what is lost in a Frequentist understanding of probability can give the impression that calibration is the fundamental goal of uncertainty quantification, leading to failures to acknowledge its limitations in practice. 

%Recognizing how a method like conformal prediction combines multiple different ``models'' can be useful for reminding us of practical considerations less often discussed in the theoretical literature.   

%\subsection{Data dependence and prioritizing theory over implementation guidance}
%To understand the value of conformal prediction for quantifying uncertainty, it can be helpful to reflect on the theory and practice of .

Another lens for thinking about epistemic uncertainty and the twoishness of methods considers what remains beyond the bounds of uncertainty quantification theory. Consider non-parametric bootstrapping, a distribution-free technique for quantifying uncertainty that resembles conformal prediction in substituting simple computations for explicit distributional assumptions.
In standard non-parametric bootstrapping, we have some observed data $\mathcal{D} = (X_{1}, \dots, X_{n}) \sim P$ and wish to quantify the uncertainty in our plug-in estimate of a ``parameter'' of $P$, $\hat{\theta}_{n}$.
Constructing valid $1-\alpha$ confidence intervals on our sample estimate means approximating the exact finite sample distribution of a test statistic involving the estimator, for example:

\begin{equation}
F_{n}(t) = \mbox{Pr}(\sqrt{n}(\hat{\theta^{*}} - \hat{\theta}_{n}) \le t)
\end{equation}
While $F_{n}$ is unknown, it can be estimated using an empirical approximation $\hat{F_{n}}$ conditional on $D$, which is treated as fixed: 
\begin{equation}
\hat{F_{n}}(t) = \mbox{Pr}(\sqrt{n}(\hat{\theta^{*}} - \hat{\theta}_{n}) \le t|X_{1},\dots,X_{n}).
\end{equation}
For this one can use the Monte Carlo approximation $\bar{F}$:
\begin{equation}
   \bar{F}(t) =  \frac{1}{B} \sum_{j=1}^{B} I(\sqrt{n}(\hat{\theta^{*}_{j}} - \hat{\theta}_{j}) \le t)
   \label{eq:bootstrap_iterations}
\end{equation}
Key ideas behind the bootstrap include the observation that an unknown probability distribution can be replaced with an empirical estimate (the substitution principle), and the use of simulation to avoid analytically calculating properties of an estimator~\citep{davison2003recent}. %Setting the number of iterations $B$ gives us a sense of control, in that with a high enough $B$ we can ignore the error induced by taking the Monte Carlo approximation $\bar{F}(t)$ to $\hat{F_{n}}$.

The twoishness of bootstrapping as a method arises from how we can think of the estimator $\hat{\theta_{n}}$ as being defined under some model (even if we treat the distribution as unknown), while the uncertainty from the sampling process is defined under a second model (the sampling distribution of the test statistic). 
Acknowledging the distinction between these two models makes clear that while the bootstrap allows us to minimize the error or uncertainty from the Monte Carlo approximation (by setting a high enough number of iterations $B$ in \ref{eq:bootstrap_iterations}, %so we can ignore the error induced by taking the Monte Carlo approximation $\bar{F}(t)$ to $\hat{F_{n}}$), 
we cannot reduce our uncertainty about how well our particular sample $\mathcal{D}$ represents $P$, and therefore our uncertainty about how well $\hat{F_{n}}$ approximates $F_{n}$. It would be a mistake to adopt the bootstrap in any particular setting without considering how the irreducible uncertainty due to having only a single sample might affect our goals, through, for example, the influence of outliers on the target statistic. 
Similarly, whenever we bring in calibration data after model training, any ``guarantees'' depend on the fitness of the calibration data as a representation of the ground truth generating process and on our ability to imagine taking hypothetical random samples of calibration and test data. 


%is of critical importance. %Reflecting on how two ``models'' are combined in the ordinary bootstrap helps draw our attention to gaps in our ability to make assurances about particular situations.

A second observation concerns a mismatch between theoretical progress in bootstrapping and the practical value of the approach. 
The ordinary bootstrap is only first-order accurate, meaning that we expect the coverage error in any particular application to scale with the square root of $n$. 
The bootstrapping literature devotes considerable attention to this question of how to improve on the first-order approximation of $F_{n}(t)$ of standard bootstrapping (e.g.,~\cite{diciccio1996bootstrap}), %is by pursuing methods that provide second-order asymptotic guarantees.  
such as by advocating the use of asymptotically pivotal statistics that converge faster than simpler alternatives (e.g., from $\mathcal{O}(n^{-1/2})$ to $\mathcal{O}(n^{-1})$; \cite{hall1994methodology}). 
However, asymptotic properties do not necessarily address the needs of practitioners concerned with singular applications governed by particular constraints. When applying bootstrapping, relevant questions concern how much data is too little to trust the resulting intervals, and what more complex dependence schemes are feasible given the amount and structure of the available data.
When applying split conformal prediction, knowing how data requirements scale may be less useful than anticipating the impacts of coverage errors and considering the tradeoffs for interpretation of conditioning guarantees differently (e.g., marginally versus on groups or labels). 


Recognizing conformalization as a model rather than a universal principle encourages the user to take care in designing the calibration set: What is the largest feasible sample size that can be obtained for the calibration set, and, if taken from data that would otherwise be used in model training, how do we expect model accuracy to be impacted? What is the appropriate level of marginalization for conditioning the guarantees given data availability and the cost of errors in the downstream decision task? These questions are not well addressed by the literature, but brushing them aside puts one at risk of quantifying prediction uncertainty performatively rather than genuinely attempting to meet the needs of decision makers.




%The guarantees afforded by bootstrapping theory do not necessarily equip a practitioner to make good decision in any single application. 
  

%Twoishness helps explain why split conformal prediction is considered so appealing. 

%Indeed, the appeal of split conformal prediction, like the broad appeal of bootstrapping, largely comes from this status as a model-agnostic wrapper framework.


%Just as asymptotics in bootstrap theory fail to explain key risks and value seen in practice, focusing on what we can prove about the coverage of split conformal prediction in expectation can lead us to overlook important gaps in guarantees that can be made in typical use.  

 % expected coverage error and the impossibility of conditional coverage.   


==> sections/notes.tex <==
\citep{straitouri2023improving}: Given estimator of expert success probability with different conformal predictors, find predictor (alpha) that maximizes gain. 

\citep{straitouri2023designing}: In this paper, we revisit the design of this type of systems from
the perspective of online learning and develop a methodology that does not require, nor assumes, an
expert model. Our methodology leverages the nested structure of the prediction sets provided by any
conformal predictor and a natural counterfactual monotonicity assumption to achieve an exponential
improvement in regret in comparison to vanilla bandit algorithms. We conduct a large-scale human
subject study (n = 2,751) to compare our methodology to several competitive baselines. 
Under the strict implementation, experts
can only predict a label value from the prediction set whereas, under the lenient implementation, experts
are encouraged to predict a label value from the prediction set but have the possibility to predict other
label values. Perhaps surprisingly, our results demonstrate that, under the strict implementation, experts
achieve higher accuracy. This suggests that, for decision support systems based on prediction sets, limiting
experts’ level of agency leads to greater performance than allowing experts to always exercise their own



\citep{de2024towards}: 
We first demonstrate that there exist (many) data distributions for which the
optimal prediction sets under which the human experts achieve the highest average accuracy cannot
be constructed using a conformal predictor. Then, we show that the problem of finding the optimal
prediction sets is NP-hard by using a reduction from the k-clique problem [22]. More strongly, unless
P = NP, we show that the problem is hard to approximate to any factor less than the size of the label
set. However, we introduce a simple and computationally efficient greedy algorithm that, for a large
class of non-conformity scores and expert models parameterized by a mixture of multinomial logit models
(MNLs), is guaranteed to find prediction sets that provably offer equal or greater performance than
those constructed using conformal prediction
